The MalSource Dataset: Quantifying Complexity and Code Reuse in Malware Development

During the last decades, the problem of malicious and unwanted software (malware) has surged in numbers and sophistication. Malware plays a key role in most of today's cyber attacks and has consolidated as a commodity in the underground economy. In this work, we analyze the evolution of malware from 1975 to date from a software engineering perspective. We analyze the source code of 456 samples from 428 unique families and obtain measures of their size, code quality, and estimates of the development costs (effort, time, and number of people). Our results suggest an exponential increment of nearly one order of magnitude per decade in aspects such as size and estimated effort, with code quality metrics similar to those of benign software.We also study the extent to which code reuse is present in our dataset. We detect a significant number of code clones across malware families and report which features and functionalities are more commonly shared. Overall, our results support claims about the increasing complexity of malware and its production progressively becoming an industry.

==> overview.tex <==
\section{Software Metrics}
\label{sec:overview}


This section provides an overview of the software metrics concepts used
in this work to quantify various aspects of malware source code. We first
introduce the two most widely used measures of software size: lines of source
code (SLOC) and function points (FP). We then introduce effort estimation
metrics, specifically the Constructive Cost Model (COCOMO), and also
measures of source code complexity and maintainability.

\subsection{Measuring Software Size}

The number of lines in the source code of a program (SLOC) constitutes
the most commonly used measure of its size. The number of physical SLOC
refers to a count of the number of lines in the source code of a program,
excluding comment and blank lines. Contrarily, logical SLOC counts take
into account language-specific aspects, such as terminating symbols and
style or formatting conventions, to deliver an estimate of the number of
executable statements. Both IEEE~\cite{IEEE93} and the Software Engineering
Institute (SEI)~\cite{Park92} had provided definitions and counting guidelines
to obtain SLOC measures.

SLOC counts have a number of shortcomings~\cite{Nguyen07} and can
be easily misused. Despite this, it has a long-standing tradition as the most
popular sizing metric. Furthermore, SLOC is an essential input for many
estimation models that aim at predicting the effort required to develop a 
system, its maintainability, the expected number of bugs/defects, or the
productivity of programmers.

Comparing size across different programming languages can give misleading
impressions of the actual programming effort: the more expressive
the programming language, the lower the size. An alternative metric
to using SLOCs as the estimated software size is to use a measure
of its functionality. The best known of such measures is the
\emph{function-point count}, initially proposed by
Albrecht~\cite{Albrecht79} and later refined by Albrecht and
Gaffney~\cite{Albrecht83}. The function-point count refers to the
overall functionality of the software and is measured by estimating
four program features: external inputs and outputs, user
interactions, external interfaces, and files used. The overall count
also involves various weights that account for the possibly different
complexity of each of the above elements. Thus, the so-called
unadjusted function-point count (UFC) is computed by simply multiplying
each count by the appropriate weight and summing up all values. The UFC
can be subsequently adjusted through various factors that are related
to the complexity of the whole system.

The expected size in SLOC of a software project can be estimated
from function-point counts through a process known as
\emph{backfiring}~\cite{Jones95}. This consists in the use of
existing empirical tables that provide the average number of SLOC
per function point in different programming languages. Software
Productivity Research (SPR)~\cite{Jones96} annually publishes such
conversion ratios for the most common programming languages in what
is known as Programming Languages Tables (PLT), which are empirically
obtained by analyzing thousands of software projects. Table~\ref{Table:SLOCFPratios}
shows the SLOC-to-function-point ratios provided by PLT v8.2 for
the languages most commonly observed in malware. Overall, backfiring
is useful as SLOC counts are not available early enough in the
requirements phase for estimating purposes. Also, the resulting UFC measure
is a more normalized measure of the source code size.


\begin{table}[h]
	\begin{center}
    \begin{tabular}{|l|r|}
      \hline
      \textbf{Programming language} & \textbf{SLOC/FP} \\
      \hline\hline
      ASP / ASP.Net & 69\\
      Assembly & 119\\
      Shell / DOS Batch & 128\\
      C & 97\\
      C\# & 54\\
      C++ & 50\\
      HTML / CSS / XML / XSLT & 34\\
      Java & 53\\
      Javascript & 47\\
      PHP & 67\\
      Pascal & 90\\
      Python & 24\\
      SQL & 21\\
      Visual Basic & 42\\
      make & 21\\
      \hline
    \end{tabular}
    \end{center}
      \caption{SLOC to function-point ratios for various programming languages.}
  \label{Table:SLOCFPratios}
\end{table}

\subsection{Effort Estimation: The Constructive Cost Model (COCOMO)}

One of the core problems in software engineering is to make an accurate
estimate of the effort required to develop a software system. This is a complex
issue that has attracted much attention since the early 1970s, resulting in
various techniques that approach the problem from different
perspectives~\cite{Sommerville06}. A prominent class of such techniques
are the so-called algorithmic cost modeling methods, which are based on
mathematical formulae that provide cost figures using as input various
measures of the program's size, organizational practices, and so on.

One of the best known algorithmic software cost estimation methods is
the Constructive Cost Model (COCOMO)~\cite{COCOMO}. COCOMO is an empirical model
derived from analyzing data collected from a large number of software
projects. These data were used to find, through basic regression,
formulae linking the size of the system, and project and team factors to
the effort to develop it. As in most algorithmic cost models, the number
of lines of source code  (SLOC) in the delivered system is the basic metric
used in cost estimation. Thus, the basic COCOMO equation for the effort
(in man-months) required to develop a software system is
\begin{equation}\label{Eq:COCOMO_Effort}
E = a_b (\mathrm{KLOC})^{b_b},
\end{equation}
where KLOC is the estimated number of SLOC expressed in thousands.
The development time (in months) is obtained from the effort as
\begin{equation}\label{Eq:COCOMO_DevTime}
D = c_b E^{d_b},
\end{equation}
and the number of people required is just
\begin{equation}\label{Eq:COCOMO_People}
P = \frac{E}{D}.
\end{equation}
In the equations above, the coefficients $a_b$, $b_b$, $c_b$, and $d_b$
are empirical estimates dependent on the type of project (see
Table~\ref{Table:COCOMOcoeffs}). COCOMO considers three types of
projects: (i) \emph{Organic} projects (small programming team, good
experience, and flexible software requirements); \emph{Semi-detached}
projects (medium-sized teams, mixed experience, and a combination of
rigid and flexible requirements); and (iii) \emph{Embedded} projects
(organic or semi-detached projects developed with tight constraints).

\begin{table}[H]
  \begin{center}
    \begin{tabular}{|l|c|c|c|c|}
      \hline
      \textbf{Software Project} & $a_b$ & $b_b$ & $c_b$ & $d_b$\\
      \hline\hline
      Organic & 2.4 & 1.05 & 2.5 & 0.38 \\
      Semi-detached & 3.0 & 1.12 & 2.5 & 0.35 \\
      Embedded & 3.6 & 1.20 & 2.5 & 0.32\\
      \hline
    \end{tabular}
  \end{center}
  \caption{Basic COCOMO coefficients.}
  \label{Table:COCOMOcoeffs}
\end{table}

The model described above is commonly known as \emph{Basic COCOMO}
and is very convenient to obtain a quick estimate of costs. A further
refinement is provided by the so-called \emph{Intermediate COCOMO}.
The main difference consists in the addition of various multiplicative
modifiers to the effort estimation ($E$) that account for attributes of
both the product and the programming process such as the expected reliability, 
and the capability and experience of the programmers.
Since these are not known for malware, 
we we will restrict ourselves to the Basic COCOMO model.


\subsection{Source Code Complexity and Maintainability}

Software complexity metrics attempt to capture properties related to the interactions between source code entities. Complexity is generally linked to maintainability, in the sense that higher levels of complexity might translate into a higher risk of introducing unintentional interactions and, therefore, software defects~\cite{Lehman96}.

One of the earliest---and still most widely used---software complexity metric is McCabe's cyclomatic complexity~\cite{McCabe76}, often denoted $M$. The cyclomatic complexity of a piece of source code is computed from its control flow graph (CFG) and measures the number of linearly independent paths within it; that is, the number of paths that do not contain other paths within themselves. Thus, a piece of code with no control flow statements has $M=1$. A piece of code with one single-condition IF statement would have $M=2$, since there would be two paths through the code depending on whether the IF condition evaluates to true or false. Mathematically, the cyclomatic complexity of a program is given by
\begin{equation}\label{Eq:CyclomaticComplexity}
M = E - N + 2P,
\end{equation}
where $E$ is the number of edges in the CFG, $N$ the number of nodes, and $P$ the number of connected components. The term ``cyclomatic'' stems from the connections between this metric and some results in graph theory and algebraic topology, particularly the so-called \emph{cyclomatic number} of a graph, which measures the dimension of the cycle space of a graph~\cite{Diestel12}.

The cyclomatic complexity has various applications in the process of developing and analyzing software products. The most direct one is to limit the complexity of the routines or modules that comprise the system. McCabe recommended that programmers should limit each module to a maximum complexity of 10,  splitting it into smaller modules whenever its complexity exceeds this value. The NIST Structured Testing Methodology~\cite{NIST96} later adopted this practice and relaxed the figure up to 15, though only occasionally and if there are well grounded reasons to do it. The cyclomatic complexity has also implications in program testing because of its connection with the number of test cases that are necessary to achieve thorough test coverage. Specifically, $M$ is simultaneously: (i) an upper bound for the number of test cases needed to achieve a complete branch coverage (i.e., to execute all edges of the CFG); and (ii) a lower bound for the number of paths through the CFG. Thus, a piece of code with high $M$ would have more pathways through the code and would therefore require higher testing effort.

\Alex{ADDRESS COMMENT 2 of REVIEWER 2:
While McCabe's complexity was introduced more than 40 years ago, it is still one of the most widely used metrics for measuring software complexity. Several authors have proposed alternative metrics based on McCabe's \cite{chidamber1994metrics}\cite{henry1981software} for measuring control flow complexity. Despite the evolution of programming language expressiveness and the quality of the development tools and environments, Cyclomatic complexity is nowadays considered able to express how defect prone a software piece is \cite{ebert2016cyclomatic}. The study of the evolution of this complexity metric has been previously explored in domains other than malicious software. For instance Warren et al. \cite{warren1999evolution} characterized the evolution of modern websites, measuring different parameters including complexity. Further, Hecht et al. included McCabe's complexity in their study regarding the changing complexity of Android applications along their evolution \cite{hecht2015tracking}.}

McCabe's . The Study of software complexity trends often resorts to cyclomatic complexity \

The cyclomatic complexity is also connected to another code metric called the maintainability index ($MI$), introduced by Oman and Hagemeister in~ \cite{Oman92}. The $MI$ is a value between 0 and 100 that measures how maintainable (i.e., easy to understand, support, and change) the source code is, with high values meaning better maintainability. One of the most common definitions of the $MI$ is given by
\begin{equation}\label{Eq:MaintainabilityIndex}
MI  = 100 \frac{171 - 5.2\ln{(\overline{V})} - 0.23 \overline{M} - 16.2 \ln{(\overline{SLOC})}}{171},
\end{equation}
where $\overline{V}$ is Halstead’s average volume per module (another classic complexity metric; see~\cite{Halstead77} for details), $\overline{M}$ is the average cyclomatic complexity per module, and $\overline{SLOC}$ is the average number of source code lines per module. The $MI$ has been included in Visual Studio since 2007 \cite{cyclomatic_visual_studio}, and in the JSComplexity and Radon \cite{metrics_radon} metrics for Javascript and Python. Although not exempt from criticisms, its use was promoted by the Software Engineering Institute in their ``C4 Software Technology Reference Guide''~\cite{STR1997} as a potentially good predictor of maintainability. As for its interpretation, there is no agreed upon safe limits. For example, Visual Studio flags as suspicious modules with $MI<20$.

